Explainable Intrusion Detection Systems Using Competitive Learning Techniques

The current state of the art systems in Artificial Intelligence (AI) enabled intrusion detection use a variety of black box methods. These black box methods are generally trained using Error Based Learning (EBL) techniques with a focus on creating accurate models. These models have high performative costs and are not easily explainable. A white box Competitive Learning (CL) based eXplainable Intrusion Detection System (X-IDS) offers a potential solution to these problem. CL models utilize an entirely different learning paradigm than EBL approaches. This different learning process makes the CL family of algorithms innately explainable and less resource intensive. In this paper, we create an X-IDS architecture that is based on DARPA's recommendation for explainable systems. In our architecture we leverage CL algorithms like, Self Organizing Maps (SOM), Growing Self Organizing Maps (GSOM), and Growing Hierarchical Self Organizing Map (GHSOM). The resulting models can be data-mined to create statistical and visual explanations. Our architecture is tested using NSL-KDD and CIC-IDS-2017 benchmark datasets, and produces accuracies that are 1% - 3% less than EBL models. However, CL models are much more explainable than EBL models. Additionally, we use a pruning process that is able to significantly reduce the size of these CL based models. By pruning our models, we are able to increase prediction speeds. Lastly, we analyze the statistical and visual explanations generated by our architecture, and we give a strategy that users could use to help navigate the set of explanations. These explanations will help users build trust with an Intrusion Detection System (IDS), and allow users to discover ways to increase the IDS's potency.

==> intro_v1.tex <==
%% main text
\section{Introduction}
\label{sec:Introduction}
The use of Artificial Intelligence (AI) in cyber-defense solutions, particularly Intrusion Detection Systems (IDS), has been gaining traction to protect against a wide range of cyber attacks. While these AI models have high detection rates, high false positive and false negative rates can dissuade a security analyst from using an AI enabled IDS %, which leads to less actionable predictions}
\cite{Marshan}. 
These IDS built using AI and deep learning methods are black boxes, meaning a security analyst will have little to no explanations and clarifications on why a model made a particular prediction. With the rise in cyber attacks on critical infrastructure, government organizations, and business networks, there is a pressing need for an explainable, automated detection system that can provide real-time aid to an analyst. 

\textcolor{red}{A potential solution to this problem is the use of Competitive Learning (CL) algorithms for intrusion detection. CL algorithms use a learning process that is different than traditional Neural Networks (NN). Where NN learn by changing weights to minimize loss, CL algorithms learn through a competitive process. This competitive process mimics data creating abstract clusters that act as feature detectors for datasets. Since the feature detectors in a CL algorithm mimic data, they can be directly compared to samples from a dataset to create various statistical and visual explanations. These explanations can then be used by stakeholders, such as Cyber-Security Operations Centers (CSoC), to help improve response time to attacks and build trust in the AI IDS.}
%{Intrusion Detection Systems are generally utilized as part of a larger cybersecurity defense effort at an organization generally located in a Cyber-Security Operations Center (CSoC).} These systems monitor networks and automate attack detection by comparing network activity to the signature of known attacks or by detecting behavior that is anomalous to benign network patterns \cite{raytheon_2017}. Through these methods, a security analyst can use an IDS to detect improper use, unauthorized access, or the abuse of a network. Analysts can then create mitigating strategies to minimize damages and costs of the malicious behavior. The usefulness and cost effectiveness of IDS have therefore been the subject of much research \cite{belouch2018performance,wu2010use}. 

\textcolor{red}{Previous AI IDS works have focused on creating highly accurate yet opaque NN models. These methods are effective at detecting anomalies, but they lack the ability to explain their reasoning. These black box NN need surrogate models to create explanations. However, surrogate models such as LIME, SHAP, and LRP do not always create useful explanations that allow for full understanding of a NN. CL algorithms, on the otherhand, are inherently explainable and allow for a plethora of customizable explanations to be generated. Not only are these models easily explainable, but they can also be just as accurate as black box NN methods. The inexplicability of Opaque Deep learning methods limits its adoption in real world cyber-defence scenarios, while highly explainable and accurate CL algorithms may be a driving factor in future Explainable Intrusion Detection System (X-IDS) solutions.  }
%Previous work in AI enabled IDS have generally focused on improving detection rates while limiting false positives and false negatives. These techniques have been effective at achieving high detection rate, but have failed to provide explanations for their computed predictions. Without the ability to understand how a model reached a decision and which features were relevant to the decision computation, a security analyst will give less credence to these AI enabled IDS. Opaque Deep Learning methods in particular, can be considered as black boxes providing no explanations and feature relevance information, severely limiting adoption in real world cyber-defense scenarios \cite{lipton2018mythos}. 

\textcolor{red}{To improve the field of X-IDS, this work uses guidelines proposed by the Defense Advanced Research Projects Agency (DARPA) to define explainable AI systems (XAI). DARPA indicates that an XAI should explain the reasoning for its decisions, characterize its strengths and weaknesses, and convey a sense of its future behavior \cite{gunning2019darpa}. An X-IDS that is transparent in its behavior and decision making process, will empower a security analyst to make better informed actions, understand the feature composition of a prediction, help CSoCs defend from known attacks, and quickly understand zero-day attacks. To address this need, an X-IDS based on Competitive Learning (CL) has been created.}

%A potential solution to this problem is to research and develop Explainable Intrusion Detection Systems (X-IDS) based on current capabilities in Explainable Artificial Intelligence (XAI) \cite{subashxids}.The guidelines proposed by the Defense Advanced Research Projects Agency (DARPA) indicate that to be explainable, an AI should explain the reasoning for its decisions, characterize its strengths and weaknesses, and convey a sense of its future behavior \cite{gunning2019darpa}. An X-IDS that is transparent in its behavior and decision making process, will empower a security analyst to make better informed actions, understand the feature composition of a prediction, help CSoCs defend from known attacks, and quickly understand zero-day attacks. To address this need, an X-IDS based on Competitive Learning (CL) has been created.

Data collected from modern networks contain potentially hundreds of different features about the traffic flow, operating systems, network protocols, and other metadata. CL learning algorithms can be used to learn patterns found in high dimensional data. SOMs, for example, learn patterns in high dimensional data and represent those patterns in a 2-dimensional plane. This creates a topographical relationship of the data by clustering similar samples closer to one another \cite{kohonen1982self}. The SOM algorithms can be taken a step further to become a Growing Self Organized Map (GSOM). Rather than having a single static map, the GSOM grows to allow for more complex patterns to be recognized. CL algorithms are further improved through the use Growing Hierarchical Self Organizing Maps (GHSOM). GHSOMs are able to create a hierarchical tree structure of multiple GSOMs, capturing more information from complex input data \cite{dittenbach2000growing}. Through SOM visualization techniques, a security analyst can view both global and local explanations about a potential attack rather than an opaque prediction generated by a black box model; however, the vertical growing process of the GHSOM can result in a structure many layers deep and consisting of 1000s of individual GSOMs. To gain understanding from such a large structure would be daunting, so a pruning process is proposed to make the exploration space more navigable and understandable for the security analyst. This process can reduce the size of the map by up to 99\% while losing little accuracy.

%Data collected from modern networks contain potentially hundreds of different features about the traffic flow, operating systems, network protocols, and other metadata. SOMs work by representing this high dimensional data on a 2-dimensional plane. This also includes maintaining the topographical relationship of the data by grouping similar data \cite{kohonen1982self}. GHSOMs go a step further and create a hierarchical tree structure of multiple SOMs, capturing more information from complex input data \cite{dittenbach2000growing}. Through SOM visualization techniques, a security analyst can view both global and local explanations about a potential attack rather than an opaque prediction generated by a black box model; however, the growing process of the GHSOM can result in a structure many layers deep and consisting of 1000s of individual SOMs. To gain understanding from such a large structure would be daunting, so a pruning process of the GHSOM will be done to make the exploration space more navigable and understandable for the security analyst.

As the need for explainable cyber-defense systems increases and to address the lack of XAI research in the field of IDS, the main objective of this paper is to create an explainable IDS that can achieve high detection accuracy. To accomplish this, we propose the use of three CL SOM algorithms to demonstrate that a higher complexity white-box algorithm is needed. Alongside this analysis, we will also provide a method for pruning large GHSOM trees to help create effective explanations. The goal of this paper is to increase trust in IDS and help CSoCs defend their networks from attacks through the use of explainable insights. 

%As the need for explainable cyber-defense systems increases and to address the lack of XAI research in the field of IDS, the main objective of this paper is to create an explainable IDS while maintaining high detection accuracy. To accomplish this the high detection accuracy  GHSOM can achieve will be used along with pruning techniques to effectively visualize the tree structure and provide explanations for why a prediction was made. The goal in this paper is to increase trust in IDS and help CSoCs defend from attack through the use of explainable insights. 

\textcolor{red}{Major contributions presented in this paper are -}
\begin{itemize}
    \item A novel X-IDS architecture featuring three CL-based algorithms, built using DARPA's proposed guidelines for an explainable system. This system is able to produce robust, explanatory visualizations for Self Organizing Map (SOM), Growing Self Organizing Map (GSOM), and Growing Hierarchical Self Organizing Map (GHSOM) models and create accurate IDS predictions.
    
    %\item A detailed discussion on the evolution of explanations generated by the SOM, GSOM, and GHSOM models. The more complex models generate varying conclusions from the data, and therefore provide more impactful explanations.
    \item A pruning process that is used to create clearer explanations from the GHSOM model. This pruning process is able to reduce the size of the GHSOM between 92\% to 99\% while losing only 0.2\% to 1.0\% accuracy.
    
    \item A performative analysis using NSL-KDD and CIC-IDS-2017. The GHSOM based model is able to achieve accuracies as high as 98.2\% on NSL-KDD and 96.7\% on CIC-IDS-2017 datasets.

    \item An analysis of statistical and visual explanations used to create an effective X-IDS architecture. Our explanation module creates a collection of explainable visualizations ranging from global significance charts to fine-grained feature explanations.
\end{itemize}

The rest of the paper is outlined as follows - In Section \ref{sec:Related Works}, we discuss some related work on IDS, XAI, and X-IDS. Section \ref{sec:Background} describes the varying CL-based algorithms used in this paper. Section \ref{sec:Architectures}, outlines our CL based X-IDS with its architecture presented in Figure \ref{fig:cl_arch}. Section \ref{sec:Experiment} discusses our experimental results. Finally, the conclusion and future work has been presented in Section \ref{sec:Conclusion}.

==> results_section_v1.tex <==
\section{Evaluation \& Experimental Results}
\label{sec:Experiment}


%\subsection{Experiment Setup}
%\label{sec:Experiment_Setup}

Our different CL based architectures and SOM variants were evaluated on both \textit{explanation generation} and \textit{traditional accuracy tests}. Experiments were run using the aforementioned datasets (See Section \ref{sec:Architectures}), which were used to train the SOM, GSOM, and GHSOM models. The SOM was setup to run over 1000 iterations using an 18 x 18 map. We found that increasing the amount of iterations served to overfit the models and decrease the overall efficacy of the model. The size of the map was chosen similarly through trial and error. The GSOM hyper parameters were set to 100 and 40 training iterations for NSL-KDD and CIC-IDS-2017 respectfully. The spread factor for these experiments was set to $.9$. This causes a very aggressive growth cycle for the neurons allowing for much quicker topological convergence. Lastly, the GHSOM hyper parameters were set to 100 epochs per SOM created with a spread factor of $.3$. These settings were discovered through the parameter optimization process outlined in Section \ref{sec:Architectures_Post-Modeling}. This section will begin by discussing the explanatory results of each of the CL models followed by the performative results.

\subsection{Visualization and Explanation}
This section will discuss the results from each of the visual and graphical explanations for all models. 

\input{local_global_explanations.tex}
    
\subsubsection{SOM Explanations}
The results for the NSL-KDD dataset can be found in Figures \ref{fig: nsl-local} and \ref{fig: nsl-global}. The local explanation example shows that the most important features for its prediction were `Duration', `Destination (dst) bytes', and `Source (src) bytes'. The remaining features, `Service (srv) count', `Count', and `Destination (dst) host count' (see Table \ref{table:feature descriptions} for descriptions) are considered less significant because of their distance from the BMU. Two of the important features coincide with the Global Feature Significance graph. This trend continues when testing on many different test samples. The most important global features are frequently at the forefront for local significance. Similarly to NSL-KDD, CIC-IDS-2017 follows this trend. Many of the top, globally selected features also play a more important role in local predictions.

The next set of explainability techniques has been data-mined from the trained SOM. Figures \ref{fig: nsl-U-Matrix} and \ref{fig: cic-U-Matrix} show the generated Starburst U-Matrix for NSL-KDD and CIC-IDS-2017, respectively. The SOM algorithm was able to separate benign clusters from malicious clusters in the map created from NSL-KDD dataset. The bottom-left corner is primarily malicious samples, while the top-right corner contains mostly benign samples. Additionally, the clusters marked by the starbursts' origins mostly represent one label. On the other hand, the CIC-IDS-2017 map has not separated the labels sufficiently. Most of the labels present in the figure are benign (0) with very few malicious labels (1). CIC-IDS-2017 is an unbalanced dataset, with about 70\% of samples being benign and 30\% of samples as malicious. This class imbalance causes the SOM to be trained on more benign samples than malicious.

Lastly, the feature value heatmaps are generated for each feature of the dataset. The examples chosen were the most significant features for each dataset: `destination (dst) bytes' and `flow bytes/s'. On their own, they can be used to see general training trends for each feature. In Figures \ref{fig: nsl-Feature} and \ref{fig: cic-Feature}, we can see that each of these features have higher values in the bottom-left units and lower values elsewhere. {Users will be able to build a mental model of the SOM when visualized in conjunction with the features maps.} For example, `destination (dst) byte', `duration', and `source (src) byte' all have higher values in the malicious section of the map. One may conclude that when these values are all close to one, the sample is more than likely malicious.


\subsubsection{GSOM Explanations}
The visualizations and explanations for GSOM are very similar to the basic SOM. Local explanations can still gained from predictions, and the global explanation for the model remains the same as it is with SOM. The U-matrix and feature component map are shown in Figure \ref{fig: GSOM-U} and Figure \ref{fig: GSOM-Feature}, respectively. A noticeable difference is the shape of the figures being irregular compared to SOM due to the fact that DBGSOMs grow directionally towards the most error. Another difference is the way neurons are depicted, as hexagons rather than squares, to better represent the irregular structure. Due to these differences, the starburst model used for SOM is, in this case, replaced by a U-matrix and a neuron label map. The label map, depicted in Figure \ref{fig: GSOM-Labels}, has the color of each hexagon representing the class label of that neuron.

\subsubsection{GHSOM Explanations}
As DBGHSOMs are comprised of a hierarchy of many different DBGSOMs, the visualizations are also more complex. Figure \ref{fig: stacked figure} shows stacked depictions of the U-matrices, feature component maps, and neuron label maps that are generated from individual DBGSOMs. The unslanted figures on the lefthand side of the figure represent the root node of the DBGHSOM. Going from left to right in the figures shows DBGSOMs deeper in the trees hierarchy. The ellipsis in the represents the amount of figures, represented beneath the ellipsis. The maps become more sparse in deeper layers of the hierarchy and the leaf nodes tend to have four neurons which is depicted on the right side of the stacked figure. 

Another method for visualizing a trained GHSOM is the treemap, which is depicted in Figure \ref{fig: treemap pruned}. This is made using the CIC-IDS dataset without utilizing the pruning method. Each larger box in the picture represents a DBGSOM with a label serving as an identifier and the layer at which it resides. Smaller boxes within the GSOM represents neurons within the GSOM and are labeled with an identifier and its size; the physical size of each neuron is based on the number of samples where that neuron is the bmu. The colors of each neuron represents the label of the neuron, unless the neuron has a child DBGSOM, in which case the identifier of the child DBGSOM is displayed on the neurons. Figure \ref{fig: treemap pruned} displays the resulting treemap of the model shown in Figure \ref{fig: treemap unpruned} after the pruning process.

\input{experiment_results.tex}

\subsection{Performative Results}
\label{sec: performative results}

The experimental results will consist of accuracy, precision, recall, f1, false positive rate, false negative rate, and network size measures. Accuracy refers to the percentage of correct predictions compared to the total test size. Precision measures the ratio of true positive predictions to the total number of positive predictions. Recall is the measure of true positives predictions to the total number of positive samples in the test set. The f1 score is a measure that gives equal weight of precision and recall. False positive rate is the rate of false positive predictions compared to the amount of ground truth negatives. False negative rate is the rate of false negative predictions compared to the amount of ground truth positives. Network size is simply the amount of GSOMs within the hierarchical GHSOM structure. For SOMs and GSOMs, the network size was 1. The training time of each algorithm and the average time for a single prediction is also measured. All results can be found in Table \ref{results table}.

\begin{comment}
Random Forest NSL-KDD \cite{farnaaz2016random}
Random Forest CICIDS-2017 \cite{goryunov2020synthesis}
DBN NSL-KDD \cite{alomDeepBelief}
DBN CICIDS-2017 \cite{belarbi2022intrusion}

\end{comment}




\subsubsection{SOM Results}

Using the settings outlined above, we can see that the accuracy of the SOM was able to achieve an accuracy of 90.7\% on NSL-KDD and 79.4\% on CIC-IDS-2017. It is notable that the model predicting for NSL-KDD has a much lower false positive rate than false negative rate. Much of the accuracy loss comes from the model mispredicting that malicious traffic is benign. What are the potential causes of this? Looking at the NSL-KDD U-matrix in Figure \ref{fig: nsl-U-Matrix}, we can see the top and bottom right clusters are well defined for malicious and benign traffic respectfully. The other starbursts have not clustered well and do not respect one label. These poorly clustered regions of the map may be the cause for the loss in accuracy. Additionally, the this model may not be able to tell the difference between regular traffic and attacks that mimic regular traffic. The amount of complexity that a SOM is able to learn is limited by its inability to grow. CIC-IDS-2017 tells a different story. Its accuracy is noticeably worse than NSL-KDD. This can be attributed to the fact that it has over-fit towards benign data. CIC-IDS-2017 is a dataset with a contamination rate of about 20\%, and with a map that cannot grow, it is difficult for it to make adjustments when malicious data is found for training. These difficulties can be easily summarized in the 55.8\% F1-score that was achieved. The model is somewhat precise but is not able to uses that precision where it matters. Lastly, it is important to note the training time of these models. The SOM is able to be quickly trained on the NSL-KDD dataset in around 8 seconds. CIC-IDS-2017 being an order of magnitude larger is noticeably slower with a training speed of 260 seconds. Both datasets achieve the same prediction speeds as map sizes are the same.
%The SOM training process consists of 1000 iterations of training on an 18x18 neuron map. For NSL-KDD, SOM obtains an accuracy of 90.7\%, precision of 97.2\%, recall of 83.3\%, F1 of 89.7\%, FPR of 2.2\%, and a FNR of 16.6\%. On CIC-IDS, the model achieves a 79.4\% accuracy, 83.2\% precision, 42.0\% recall, 55.8\% F1 score, 19.0\% FPR, and a 23.0\% FNR.

\subsubsection{GSOM Results}

The Growing SOM, on the other hand, is able to achieve far greater results than its predecessor. On the NSL-KDD dataset, it is able to achieve an accuracy of 96.0\%. It is also able to reduce the amount of false negatives while gaining a small amount of false positives from the previous model. This increased performance can be attributed to the growing nature of the GSOM. As new data, benign or malicious, is found, the map is able to expand itself to allow for new ideas to be learned. Viewing the NSL-KDD map in Figure \ref{fig: GSOM-U}, we can see this premise in action. On the left side of the map, there are long rows of nodes that have been added. This kind of stretching shows that there are properties in attacks that are similar to one another, but different enough to need expansion. Had these expansion not been allowed, there is a chance that nodes closer to the center of the map could have been overwritten or had their original prediction idea clouded. Figure \ref{GSOM-Vis-cic} depicts the visualizations generated from DBGSOM after training on the CIC-IDS-2017 dataset. The accuracy results for CIC-IDS-2017 are interesting. The model is able to achieve an accuracy of 95.1\% even though the neuron label display 10 clear malicious nodes. The model may be overfit towards benign data just like its SOM counterpart, so better preprocessing or a more refined training process could be used to increase detection rates. The increased detection rates of the GSOM do come with a small performative cost. It takes about 10 times longer to train a GSOM instead of a SOM. However, once trained, the GSOM is able to make predictions at the same speed as a SOM. 
%For NSL-KDD, the DBGSOM was trained for 100 epochs with a spreading factor of .9 causing an aggressive growth of neurons and quicker topological convergence. This model achieved and accuracy of accuracy of 96.0\%, precision of 96.9\%, recall of 94.7\%, F1 of 95.8\%, FPR of 2.9\%, and a FNR of 5.2\%. CIC-IDS was trained over 40 epochs and a spreading factor of .9 and resulted in a 95.1\% accuracy, 84.8\% precision, 91.3\% recall, 87.9\% F1 score, 4.0\% FPR, and a 8.7\% FNR.

\input{figures/tex_files/ghsom_pruning_figure.tex}

\subsubsection{GHSOM Results}

Out of all of the models, our GHSOM models were able to achieve the best results. The results from these models can be divided into regular and pruned. The regular models were able to achieve the highest results of 98.2\% on NSL-KDD and 96.7\% on CIC-IDS-2017. The pruned results take a minor decrease to their accuracies of 98.0\% and 95.7\% respectfully. The increased detection rates over the previous two CL algorithms can be attributed to the GHSOM's more complex learning style. Vertical growth is able to help divide benign and malicious traffic. We can see this in the regular and pruned visualizations (\ref{fig: treemap unpruned} \& \ref{fig: treemap pruned}). On the left side of the figures we see more of the leaf nodes. If we view the pruned CIC-IDS-2017 figure, many of these branches of nodes appear to respect one type of label. The performative loss for the GHSOM comes at an order of magnitude for both regular and pruned GHSOMs. 
%The DBGHSOM for NSL-KDD was again trained for 100 epochs but at a lower spreading factor of .3. This causes the root map to grow less and allows for more of the hierarchies of the input data to be captured in lower layers and branches of the the tree. This model obtained a 98.2\% accuracy, 98.0\% precision, 98.3\% recall, 98.1\% F1 score, 1.9\% FPR, and a 1.6\% FNR. The network size was 7288 total GSOMs. Pruning this model with a $\delta$ of 10 and a c value of .3 reduced the size of the network to 574 and maintained an accuracy of 98.0\%, precision of 98.0\%, recall of 97.8\%, F1 of 97.9\%, FPR of 1.8\%, and a FNR of 2.2\%. 

%The DBGHSOM trained on CIC-IDS also has a lower spreading factor of .3 to allow for more vertical growth rather than horizontal growth. It was trained over 40 epochs and resulted in an accuracy of 96.7\%, precision of 89.1\%, recall of 94.5\%, F1 of 91.7\%, FPR of 2.8\%, FNR of 5.5\%, and a network size of 16894. Pruning with the same parameters used to prune the NSL-KDD model reduced the network size to 119. This model achieved an accuracy of 95.7\%, precision of 86.5\%, recall of 92.7\%, F1 of 89.5\%, FPR of 3.5\%, FNR of 7.3\%



\section{Discussion}

For all models, Figure \ref{fig: local-global} shows the local explanations that are made for predictions and the global importance variables have when creating the models. The following subsections will discuss the unique visualizations generated from each model, the quality of explanations they produce, and how they can be used with the local and global explanations to gain understanding about the input data and predictions made. Lastly, we will compare the performative results from each of the CL models.

\input{figures/tex_files/som_local_global.tex}

\subsubsection{SOM}
When analyzing the starburst matrix in Figure \ref{fig: nsl-U-Matrix} and Figure \ref{fig: cic-U-Matrix}, each neuron is labeled with the class label used when making predictions. Observing the neurons close to each other, denoted as darker areas in the map, along with class labels gives information about areas of the data that are closely associated with malicious network behavior. For NSL-KDD, the top right corner of the map is an area of interest because all of that area's neurons are labeled as malicious. Used in conjunction with global and local explanations, important features such as `destination (dst) bytes' can be observed in Figure \ref{fig: nsl-Feature}. This comparison shows a correlation with high `dst bytes' values and the neuron cluster with malicious labels. One can go further looking at other important feature component maps to gain a more complete picture of why the model came to a certain prediction. Users will be able to build a mental model of the SOM when visualized in conjunction with the feature maps. For example, if `dst byte', `duration', and `source (src) byte' all have higher values in the malicious section of the map then One may conclude that when these values are all close to one, the sample is more than likely malicious.

The same kind of explanations can be gained from the SOM model trained on CIC-IDS. In this case, however, the SOM algorithm is inadequate in modeling the input data and does not provide high quality visualizations. Nearly all neurons are labeled as benign with a small amount of neurons labeled as malicious spread throughout the map. CIC-IDS-2017 is an unbalanced dataset, with about 70\% of samples being benign and 30\% of samples as malicious. This class imbalance causes the SOM label neurons as benign rather than malicious.



\input{figures/tex_files/gsom_explanations.tex}

\subsubsection{GSOM}
Visualizations and explanations garnered from GSOMs are very similar. But due to the irregular nature of the models, the starburst model from SOM is replaced with a U-matrix and label map. The label map in this case does appear easier to read and compare to the other maps as the neurons are brightly colored to denote class while the class labels on the starburst U-matrix blend in and are harder to read. Figure \ref{GSOM Visualizations} shows the visualizations created from training on NSL-KDD. Comparing the label map in Figure \ref{fig: GSOM-Labels} and the feature component map in Figure \ref{fig: GSOM-Feature} shows an interesting deviation from the explanations generated from the SOM visualizations. Here low `dst byte' values correlate to malicious network traffic, the opposite of the conclusion drawn from the SOM model. Here the GSOM saw a higher potential in low `dst byte' values and ended up being more trustworthy with higher accuracy scores than the SOM model.



\subsubsection{GHSOM}
The visualizations created for GHSOM are inherently the same, but a single model is made up of a hierarchy of multiple GSOM visualizations. Figure \ref{fig: stacked figure} shows the stacked U-matrices, feature maps, and label maps. GHSOM provides a highly accurate model at the cost of the simplicity of the model, though this may be preferable to a security analyst who is exploring the intricacies of a complex dataset. To gain a local explanation, a security analyst can dig into the hierarchy to the GSOM that made the classification and explore the properties of those visualizations. While this maybe useful to find different hierarchies of the data, a GHSOM grown too large become to complex for anyone to understand. Figure \ref{fig: treemap unpruned} shows a tree-map of a model trained on CIC-IDS, and while making sense of the root and upper layers may be feasible, the lower layers and branches are so numerous that a cogent analysis of the model would be impossible. 

Pruning of the GHSOM maintains a model which captures the complexity of the data, is highly accurate, and can be easily explored. And while the training time for the pruned GHSOM is much higher than than the unpruned GHSOM, the time saved per prediction from 1.15 ms to .03 ms saves time in the long run for an extensively used model. Figure \ref{fig: treemap pruned} demonstrates the tree-map from Figure \ref{fig: treemap unpruned} after undergoing pruning. Compared to the unpruned tree-map, there are many more visible GSOMs that can be explored by visualizing the size and classes of the neurons in each GSOM and by using the GSOM identifiers to analyze the visualizations from Figures \ref{fig:1}, \ref{fig:2}, and \ref{fig:3}. There are GSOMs with mostly benign and a with a few malicious neurons that a security analyst can use to understand network traffic that is close to being benign but is actually malicious. On the other hand, there are some GSOMs in the tree-map that consist of mostly malicious neurons with a few benign neurons. This could be analyzed to flag possible false negative predictions as a possible threat. GSOMs that are entirely malicious or benign can be used to understand the intricacies of different types of malicious and benign behavior.



\subsection{Model Performance}
Similar trends between the NSL-KDD models and CIC-IDS models can be seen when comparing results from Table \ref{results table}. SOMs tend to perform the worst with a severe drop in accuracy and an increased false positive and negative rate for both NSL-KDD and CIC-IDS. The GSOM models offer competitive performance to the hierarchical models but with slightly less performance but with the benefit of containing all of the information in one self-contained map. GHSOMs provide the highest performance around the board with decreased false positive rates and false negative rates along with higher accuracy measures. They do have a very high network size however with the models trained on both datasets having thousands of GSOM nodes. The pruned GHSOM for NSL-KDD has only a slight decrease in accuracy measures and slight increases in classification rates while also reducing the network size significantly from 7288 nodes to 574 nodes. The decrease in accuracy for the pruned model trained on CIC-IDS-2017 is greater, but the reduction in network size was much greater, dropping it from 16894 nodes to 119 nodes. A less aggressive pruning process may have maintained the accuracy of the model while still reducing the network size by a significant amount. 

==> results_section_v2.tex <==
\section{Evaluation \& Experimental Results}
\label{sec:Experiment}

Our CL based architecture and its SOM variants were evaluated on both \textit{explanation generation} and \textit{traditional performative tests}. The datasets used to test our architecture were NSL-KDD and CIC-IDS-2017 (see Section \ref{sec:Architectures_Pre-Modeling}). Explanations generated for our testing include statistical and visual variants that are used by the user to complete a task. Performative metrics are recorded that allow our explainable architecture to be compared to others in the literature.

%Performative tests allow us to compare our architecture to others in the literature. 

The parameters selected for our models can be found in Table \ref{table: parameters}. In this work, the SOM was setup to run over 1000 epochs using an 18 $x$ 18 map. We found that increasing the number of epochs served to overfit the models and decrease the overall efficacy of the model. Both the size of the map and the number of training epochs were chosen through trial and error. The GSOM parameters were set to 100 and 40 training epochs for NSL-KDD and CIC-IDS-2017 respectively. We found that this in addition to an aggressive Spread Factor (SF) of .9 created the best performative results. The GHSOM parameters where set to 100 epochs per GSOM created using a SF of .3 and a Learning Rate (LR) of .006. These settings were discovered using the parameter selection process outlined in Section \ref{sec:Architectures_Post-Modeling}. This section will begin by analyzing the explanatory graphics created by the architecture followed by a discussion on the performative results.

\subsection{Visualization and Explanation}
In the final phase of our architecture, visual and statistical explanations are generated for the user. Each of the CL models uses the same local and global statistical explanations but has a tailored visual explanation.

\input{local_global_explanations.tex}

\subsubsection{SOM Explanations}
The statistical explanations for the NSL-KDD dataset can be found in Figures \ref{fig: nsl-local} and \ref{fig: nsl-global}. The local explanation example shows that the most important features for its prediction were `Duration', `Destination (dst) bytes', and `Source (src) bytes'. The remaining features, `Service (srv) count', `Count', and `Destination (dst) host count' (see Table \ref{table:feature descriptions} for descriptions) are considered less significant because of their distance from the BMU. Two of the important features coincide with the Global Feature Significance graph. This trend continues when testing on many different test samples. The most important global features are frequently at the forefront of local significance. Similarly to NSL-KDD, CIC-IDS-2017 follows this trend. Its local and global explanations can be found in Figures \ref{fig: cic-local} and \ref{fig: cic-global}. Many of the top, globally selected features also play a more important role in local predictions.

The next explainability technique has been data-mined from the trained SOM. Figures \ref{fig: nsl-U-Matrix} and \ref{fig: cic-U-Matrix} show the generated Starburst U-Matrix \cite{yuan2018implementation} for NSL-KDD and CIC-IDS-2017, respectively. The SOM algorithm was able to separate benign clusters from malicious clusters in the map created from the NSL-KDD dataset. The top-right corner is primarily malicious samples, while the bottom-right corner contains mostly benign samples. Additionally, the clusters marked by the starbursts' origins mostly represent one label. On the other hand, the CIC-IDS-2017 map has not separated the labels sufficiently. Most of the labels present in the figure are benign (0) with very few malicious labels (1). CIC-IDS-2017 is an unbalanced dataset, with about 70\% of the samples being benign and 30\% of samples as malicious. This class imbalance causes the SOM to be trained on more benign samples than malicious.

Lastly, the feature value heatmaps are generated for each feature of the dataset. The examples chosen were the most significant features for each dataset: `destination (dst) bytes' and `flow bytes/s'. On their own, they can be used to see general training trends for each feature. In Figures \ref{fig: nsl-Feature} and \ref{fig: cic-Feature}, we can see that each of these features have higher values in the bottom-left units and lower values elsewhere. {Users will be able to build a mental model of the SOM when visualized in conjunction with the features maps.} %For example, if `destination (dst) byte', `duration', and `source (src) byte' all have higher values in the malicious section of the map. One may conclude that when these values are all close to one, the sample is more than likely malicious.

\input{figures/tex_files/som_local_global.tex}

\textit{SOM Explanation Discussion:} When analyzing the starburst matrices in Figure \ref{fig: nsl-U-Matrix} and Figure \ref{fig: cic-U-Matrix}, each neuron is labeled with a class used when making predictions. Observing the darker areas that respect one label along with the feature heatmaps can give one insight into malicious behaviour.
%Observing the neurons close to each other, denoted as darker areas in the map, along with class labels gives information about areas of the data that are closely associated with malicious network behavior. 
For NSL-KDD, the top right corner of the map is an area of interest because all of that area's neurons are labeled as malicious. Used in conjunction with global and local explanations, important features such as `destination (dst) bytes' can be observed in Figure \ref{fig: nsl-Feature}. This comparison shows a correlation with high `dst bytes' values and the neuron cluster with malicious labels. One can go further looking at other important feature component maps to gain a more complete picture of why the model came to a certain prediction.  For example, if `dst byte', `duration', and `source (src) byte' all have higher values in the malicious section of the map then one may conclude that when these values are all close to one, the sample is more than likely malicious. Unfortunately, the same analysis cannot be done for the CIC-IDS-2017 model. The class imbalance has caused the model to overfit towards benign data. In this instance, one of the users could modify the preprocessing for this dataset. A stratified sampling method may prove beneficial to improving the model's explanatory and performative results.


\input{figures/tex_files/gsom_explanations.tex}

\subsubsection{GSOM Explanations}
\hl{paragraph or some sentences detailing local and global expl}

%The visualizations and explanations for GSOM are very similar to the basic SOM. Local explanations can still be gained from predictions, and the global explanation for the model remains the same as it is with SOM. The U-matrix and feature component map are shown in Figure \ref{fig: GSOM-U nsl-kdd} and Figure \ref{fig: GSOM-Feature nsl-kdd}, respectively. A noticeable difference is the shape of the figures being irregular compared to SOM due to the fact that GSOMs grow directionally towards the most error. Another difference is the way neurons are depicted, as hexagons rather than squares, to represent the irregular structure better. Due to these differences, the starburst model used for SOM is, in this case, replaced by a U-matrix and a neuron label map. The label map, depicted in Figure \ref{fig: GSOM-Labels nsl-kdd}, has the color of each hexagon representing the class label of that neuron.

The visual explanations for the GSOM can be viewed in Figure \ref{GSOM Visualizations}. It consists of the same type of visualizations that the SOM uses. However, due to the GSOM's growing nature, we are unable to use the Starburst U-matrix. We found that using hexagonal grid helped to better represent the GSOM's irregular structure. Additionally, a label map was created to represent class labels for the model. The NSL-KDD figures contain some interesting results. Firstly, the U-matrix shows several dense zones of nodes. There appear to be two clusters that are associated with malicious traffic. The main one being at the bottom-left. We also see that some clusters grow outward with single node expansions. This is because the GSOM grows directionally towards the highest error. This may mean that many of the different attack types have merged together in the bottom-left of the map. CIC-IDS-2017, however, has had the opposite experience. It has created a more homogeneous grouping of nodes. Since most of the CIC-IDS-2017's dataset is normal traffic, the map appears to grow on all sides evenly. One may conclude the the model is overfitted as there is only one section of maliciously labeled nodes. However, the performative results show that even with a small number of malicious nodes, the model performs well.

\textit{GSOM Explanation Discussion:} Visualizations and explanations garnered from GSOMs are very similar. Comparing the label map in Figure \ref{fig: GSOM-Labels nsl-kdd} and the feature component map in Figure \ref{fig: GSOM-Feature nsl-kdd} shows an interesting deviation from the explanations generated from the SOM visualizations. Here low `dst byte' values correlate to malicious network traffic, the opposite of the conclusion drawn from the SOM model. The GSOM saw a higher potential in low `dst byte' values and ended up being more trustworthy with higher accuracy scores than the SOM model. Similarly to the SOM, a user can then check other feature value heatmaps to generate their own mental model of the GSOM.

The explanatory results for CIC-IDS-2017 GSOM are also very interesting. The model was able to achieve better performative results than the SOM while labeling only a small portion of nodes malicious. This can be seen in Figure \ref{fig: GSOM-Labels cic-ids}. One would expect the false positive rate to be much higher.  Figure \ref{fig: GSOM-U cic-ids} shows some separation in clusters, however these clusters appear to be variations of benign data. Although this model has decent performative results, its explanations appear lacking. This showcases one of the many reasons a user may want to modify the architecture. In this case, the user may want to take similar action to the SOM. Preprocessing the dataset to make it train on less benign data may make its explanations more useful. Alternatively, modifying the parameters or simply creating a new model may also create better explanation.

\subsubsection{GHSOM Explanations}
Similar to the previous two methods, GHSOMs benefit from the same statistical local and global explanations. Locally, \hl{talk about the local explanation bar chart}. 


As GHSOMs are comprised of a hierarchy of many different GSOMs, the visualizations are also more complex. Figure \ref{fig: stacked figure} shows stacked depictions of the U-matrices, feature component maps, and neuron label maps that are generated from individual GSOMs. The unslanted figures on the lefthand side of the figure represent the root node of the GHSOM. Going from left to right in the figures shows GSOMs deeper in the tree's hierarchy. The ellipsis represents the number of figures, represented beneath the ellipsis. The maps become more sparse in deeper layers of the hierarchy and the leaf nodes tend to have four neurons which is depicted on the right side of the stacked figure. 

\hl{I believe this needs more clarification}
Another method for visualizing a trained GHSOM is the treemap, which is depicted in Figure \ref{fig: treemap pruned}. This is made using the CIC-IDS dataset without utilizing the pruning method. Each larger box in the picture represents a GSOM with a label serving as an identifier and the layer at which it resides. Smaller boxes within the GSOM represent neurons within the GSOM and are labeled with an identifier and its size; the physical size of each neuron is based on the number of samples where that neuron is the bmu. The colors of each neuron represent the label of the neuron, unless the neuron has a child GSOM, in which case the identifier of the child GSOM is displayed on the neurons. Figure \ref{fig: treemap pruned} displays the resulting treemap of the model shown in Figure \ref{fig: treemap unpruned} after the pruning process.

\textit{GHSOM Explanation Discussion:} The visualizations created for GHSOM are inherently the same, but a single model is made up of a hierarchy of multiple GSOM visualizations. Figure \ref{fig: stacked figure} shows the stacked U-matrices, feature maps, and label maps. GHSOM provides a highly accurate model at the cost of the simplicity of the model, though this may be preferable to a security analyst who is exploring the intricacies of a complex dataset. To gain a local explanation, a security analyst can dig into the hierarchy to the GSOM that made the classification and explore the properties of those visualizations. While this maybe useful to find different hierarchies of the data, a GHSOM grown too large become to complex for anyone to understand. Figure \ref{fig: treemap unpruned} shows a tree-map of a model trained on CIC-IDS, and while making sense of the root and upper layers may be feasible, the lower layers and branches are so numerous that a cogent analysis of the model would be impossible. 

Pruning of the GHSOM maintains a model which captures the complexity of the data, is highly accurate, and can be easily explored. And while the training time for the pruned GHSOM is much higher than than the unpruned GHSOM, the time saved per prediction from 1.15 ms to .03 ms saves time in the long run for an extensively used model. Figure \ref{fig: treemap pruned} demonstrates the tree-map from Figure \ref{fig: treemap unpruned} after undergoing pruning. Compared to the unpruned tree-map, there are many more visible GSOMs that can be explored by visualizing the size and classes of the neurons in each GSOM and by using the GSOM identifiers to analyze the visualizations from Figures \ref{fig:1}, \ref{fig:2}, and \ref{fig:3}. There are GSOMs with mostly benign and a with a few malicious neurons that a security analyst can use to understand network traffic that is close to being benign but is actually malicious. On the other hand, there are some GSOMs in the tree-map that consist of mostly malicious neurons with a few benign neurons. This could be analyzed to flag possible false negative predictions as a possible threat. GSOMs that are entirely malicious or benign can be used to understand the intricacies of different types of malicious and benign behavior.



\input{experiment_results.tex}

\subsection{Performative Results}
\label{sec: performative results}

The performative results will consist of accuracy, precision, recall, f1, false positive rate, false negative rate, and network size measures. Accuracy refers to the percentage of correct predictions compared to the total test size. Precision measures the ratio of true positive predictions to the total number of positive predictions. Recall is the measure of true positives predictions to the total number of positive samples in the test set. The f1 score is a measure that gives equal weight of precision and recall. False positive rate is the rate of false positive predictions compared to the amount of ground truth negatives. False negative rate is the rate of false negative predictions compared to the amount of ground truth positives. Network size is simply the amount of GSOMs within the hierarchical GHSOM structure. For SOMs and GSOMs, the network size was 1. The training time of each algorithm and the average time for a single prediction is also measured. All results can be found in Table \ref{results table}.

\begin{comment}
Random Forest NSL-KDD \cite{farnaaz2016random}
Random Forest CICIDS-2017 \cite{goryunov2020synthesis}
DBN NSL-KDD \cite{alomDeepBelief}
DBN CICIDS-2017 \cite{belarbi2022intrusion}

\end{comment}




\subsubsection{SOM Results}

Using the settings outlined in Table \ref{table: parameters}, we can see that the SOM was able to achieve an accuracy of 90.7\% on NSL-KDD and 79.4\% on CIC-IDS-2017. It is notable that the model predicting for NSL-KDD has a much lower false positive rate than false negative rate. Much of the accuracy loss comes from the model mispredicting that malicious traffic is benign. What are the potential causes of this? Looking at the NSL-KDD U-matrix in Figure \ref{fig: nsl-U-Matrix}, we can see the top and bottom right clusters are well defined for malicious and benign traffic. The other starbursts have not clustered well and do not respect one label. These poorly clustered regions of the map may be the cause for the loss in accuracy. Additionally, the model may not be able to tell the difference between regular traffic and attacks that mimic regular traffic. The amount of complexity that a SOM is able to learn is limited by its inability to grow. CIC-IDS-2017 tells a different story. Its accuracy is noticeably worse than NSL-KDD. This can be attributed to the fact that it has overfit towards benign data. CIC-IDS-2017 is a dataset with a contamination rate of about 20\%, and with a map that cannot grow, it is difficult for it to make adjustments when malicious data is found for training. These difficulties can be easily summarized in the 55.8\% F1-score that was achieved. Lastly, it is important to note the training time of these models. The SOM is able to be quickly trained on the NSL-KDD dataset in around 8 seconds. CIC-IDS-2017 being an order of magnitude larger is noticeably slower with a training speed of 260 seconds. Both datasets achieve the same prediction speeds because map sizes are the same.
%The SOM training process consists of 1000 iterations of training on an 18x18 neuron map. For NSL-KDD, SOM obtains an accuracy of 90.7\%, precision of 97.2\%, recall of 83.3\%, F1 of 89.7\%, FPR of 2.2\%, and a FNR of 16.6\%. On CIC-IDS, the model achieves a 79.4\% accuracy, 83.2\% precision, 42.0\% recall, 55.8\% F1 score, 19.0\% FPR, and a 23.0\% FNR.

\subsubsection{GSOM Results}

The Growing SOM, on the other hand, is able to achieve far greater results than its predecessor. On the NSL-KDD dataset, it is able to achieve an accuracy of 96.0\%. It is also able to reduce the number of false negatives while gaining a small number of false positives from the previous model. This increased performance can be attributed to the growing nature of the GSOM. As new data, benign or malicious, is found, the map is able to expand itself to allow for new ideas to be learned. Viewing the NSL-KDD map in Figure \ref{fig: GSOM-U nsl-kdd}, we can see this premise in action. On the left side of the map, there are long rows of nodes that have been added. This kind of stretching shows that there are properties in attacks that are similar to one another, but different enough to need expansion. Had these expansions not been allowed, there is a chance that nodes closer to the center of the map could have been overwritten or had their original prediction idea clouded. Figure \ref{fig: GSOM-U cic-ids} depicts the visualizations generated from GSOM after training on the CIC-IDS-2017 dataset. The accuracy results for CIC-IDS-2017 are interesting. The model is able to achieve an accuracy of 95.1\% even though the neuron label display 10 clear malicious nodes. The model may be overfitted towards benign data just like its SOM counterpart, so better preprocessing or a more refined training process could be used to increase detection rates. The increased detection rates of the GSOM do come with a small performative cost. It takes about 10 times longer to train a GSOM instead of a SOM. However, once trained, the GSOM is able to make predictions at the same speed as a SOM. 
%For NSL-KDD, the DBGSOM was trained for 100 epochs with a spreading factor of .9 causing an aggressive growth of neurons and quicker topological convergence. This model achieved and accuracy of accuracy of 96.0\%, precision of 96.9\%, recall of 94.7\%, F1 of 95.8\%, FPR of 2.9\%, and a FNR of 5.2\%. CIC-IDS was trained over 40 epochs and a spreading factor of .9 and resulted in a 95.1\% accuracy, 84.8\% precision, 91.3\% recall, 87.9\% F1 score, 4.0\% FPR, and a 8.7\% FNR.

\input{figures/tex_files/ghsom_pruning_figure.tex}

\subsubsection{GHSOM Results}

The results from these models can be divided into regular and pruned. The regular models were able to achieve the highest results of 98.2\% on NSL-KDD and 96.7\% on CIC-IDS-2017. The pruned results take a minor decrease to their accuracies of 98.0\% and 95.7\%. The increased detection rates over the previous two CL algorithms can be attributed to the GHSOM's more complex learning style. Vertical growth is able to help divide benign and malicious traffic. We can see this in the regular and pruned visualizations (\ref{fig: treemap unpruned} \& \ref{fig: treemap pruned}). On the left side of the figures we see more of the leaf nodes. If we view the pruned CIC-IDS-2017 figure, many of these branches of nodes appear to respect one type of label. The performative loss for the GHSOM comes at an order of magnitude for both regular and pruned GHSOMs. The SOM and GSOM have

%Out of all of the models, our GHSOM models were able to achieve the best performative results. The architecture is able to achieve accuracies of 98.2\% on NSL-KDD and 96.7\% on CIC-IDS-2017. The pruned model is also able to achieve high accuracies of 98.0\% and 95.7\%. Compared to the other models, the explanations are an area that need more work. Its explanations can be confusing to look at because of its large number of nodes. The GSOM and SOM have much easier to read explanations that allow the user to more easily create a mental map of the model. The performative and explanatory results for these models may be improved by applying different preprocessing techniques. Overall, the CL models used in this experiment show great promise in the area of X-IDS

\subsubsection{Model Performance Discussion}
Similar trends between the NSL-KDD models and CIC-IDS models can be seen when comparing results from Table \ref{results table}. SOMs tend to perform the worst with a severe drop in accuracy and an increased false positive and negative rate for both NSL-KDD and CIC-IDS. The GSOM models offer competitive performance to the hierarchical models but with slightly less performance but with the benefit of containing all of the information in one self-contained map. GHSOMs provide the highest performance around the board with decreased false positive rates and false negative rates along with higher accuracy measures. They do have a very high network size however with the models trained on both datasets having thousands of GSOM nodes. The pruned GHSOM for NSL-KDD has only a slight decrease in accuracy measures and slight increases in classification rates while also reducing the network size significantly from 7288 nodes to 574 nodes. The decrease in accuracy for the pruned model trained on CIC-IDS-2017 is greater, but the reduction in network size was much greater, dropping it from 16894 nodes to 119 nodes. A less aggressive pruning process may have maintained the accuracy of the model while still reducing the network size by a significant amount. 

==> tableexample.tex <==

\begin{table}
    \begin{tabularx}{0.45\textwidth} { 
      | >{\centering\arraybackslash}p{0.08\textwidth}|X
      | >{\raggedright\arraybackslash}X | }
        \hline
            \textbf{Symbol} &  \textbf{Meaning} \\
        \hline
            $IRS_{ia}$ & The intermediate action from the Plan IRS component. \\
        \hline
            $IRS_{t}$ & The target resource (e.g. "/products" webpath or a file system path) of the $IRS_{ia}$ \\ 
        \hline
            $IRS_{s}$ & The source of the $IRS_{ia}$ \\ 
        \hline
            $IRS_{ip}$ & The intermediate plan from the Plan IRS component containing $\{IRS_{ia}\}$. \\
        \hline
            $IRS_{ia_{params}}$ & The parameters such as source, target, etc. of an $IRS_{ia}$ i.e. \{$IRS_s$, $IRS_t$\} \\
        \hline
            $IRS_{res_{input}}$ & The input such as action, source, target, etc. of an $IRS_{ia}$ i.e. \{$IRS_{ia}$, $IRS_{ia_{params}}$\} \\
        \hline
            $IRS_{res_{output}}$ & The evaluated action of $IRS_{res_{input}}$ i.e.  \{$IRS_{a}$\} \\
        \hline
            $IRS_{a}$ & The RoE evaluated final action corresponding of  $IRS_{ia}$ \\
        \hline
            $IRS_{p}$ & The final plan from the RES IRS component containing $\{IRS_{a}\}$. \\
        \hline
            $RoE_{r}$ & A generic RoE rule. \\
        \hline
            $RoE_{r}^{i}(j)$ & A specific RoE rule of a specific managed system. \\
        \hline
            $RoE$ & Set of all rules i.e. $\{RoE_{r}\}$ \\  
        \hline
            $r_{a}$ & Antecedent of a $RoE_{r}$. \\ 
        \hline
            $r_{p}$ & Precedent of a $RoE_{r}$. \\ 
        \hline
            $r_{id}$ & A unique id for the rule $RoE_{r}$. \\ 
        \hline
            $r_{s}$ & The anticipated source type $RoE_{r}$ (e.g. username or IP) \\ 
        \hline
            $r_{v}$ & The $IRS_{ia}$ intended action (e.g. create, read, update, delete) \\
        \hline
            $r_{scope}$ & The target scope of $IRS_{ia}$ \\
        \hline
            $r_{c}$ & The constraint applied to the $IRS_{ia}$ (e.g. allow, deny) \\  
        \hline
            $r_{a}$ & The RoE evaluated action corresponding to $IRS_{ia}$ \\
        \hline
            $r_{f}$ & An optional handler to handle complex and custom RoE evaluation for $IRS_{ia}$ \\
        \hline
            $IRS_{D}^i$ & It is a standard deny action for a managed system for example, for a 'denied' constraint rule. \\
        \hline
            $RoE_{t}$ & A meta template that each domain \{$RoE_{t}^{i}$\} follows and ultimately all $RoE_{r}$ are compliant to.\\
        \hline
            $RoE_{t}^{i}$ & A template for a specific managed system that each $RoE_{r}^{1}(j)$ of \{$RoE_{r}$\} follows \\    
        \hline  
    \end{tabularx}
    \caption{Main notation used in this paper.}
    \label{tbl:notation-table}
\end{table}

